Exact Combinatorial Optimization with Temporo-Attentional Graph Neural Networks

Combinatorial optimization finds an optimal solution within a discrete set of variables and constraints. The field has seen tremendous progress both in research and industry. With the success of deep learning in the past decade, a recent trend in combinatorial optimization has been to improve state-of-the-art combinatorial optimization solvers by replacing key heuristic components with machine learning (ML) models. In this paper, we investigate two essential aspects of machine learning algorithms for combinatorial optimization: temporal characteristics and attention. We argue that for the task of variable selection in the branch-and-bound (B&B) algorithm, incorporating the temporal information as well as the bipartite graph attention improves the solver's performance. We support our claims with intuitions and numerical results over several standard datasets used in the literature and competitions. Code is available at: https://developer.huaweicloud.com/develop/aigallery/notebook/detail?id=047c6cf2-8463-40d7-b92f-7b2ca998e935

==> sections/extra.tex <==
\begin{table}[]
    \centering
\scriptsize
{
    \begin{tabular}{c}
        Dual Integral Reward for Different Time Limits \\
         \Xhline{2\arrayrulewidth}
    \begin{tabular}{l|cccccccc}
        \backslashbox{Method}{Time}& 60s&120s&240s&480s&900s&1200s&2400s&3600s\\    
         \Xhline{1\arrayrulewidth}
         FSB&   16,312&	32,672&	65,430&	131,607&	247,929&	332,269&	669,657&	1,011,084  \\
         
         \Xhline{1\arrayrulewidth}
         PSE&16,305&	32,671&	65,432&	131,717&	248,820&	333,024&	672,649&	1,017,046\\   
         RND&   16,459&	33,130&	66,835&	134,991&	254,630&	341,881&	690,202&	1,040,238  \\
         GCNN&  16,362&	32,826&	66,109&	133,572&    253,731&    340,771&    693,686&	1,048,019\\
         \Xhline{2\arrayrulewidth}
         TGAT&  17,295&	34,939&	70,492&	142,248&	268,781&	359,742&	725,108&	1,092,453
    \end{tabular}
        \end{tabular}
    \caption{Dual Integral Reward for Set Covering Dataset}
    \label{tab:reward_setcover}
}
\end{table}

\begingroup
\setlength{\tabcolsep}{6pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
\begin{table}[]
\scriptsize
{
    \centering
    \begin{tabular}{c}
        Dual Integral Reward for Different Time Limits \\
         \Xhline{2\arrayrulewidth}
        \begin{tabular}{l|cccccccc}
            \backslashbox{Method}{Time}& 60s&120s&240s&480s&900s&1200s&2400s&3600s\\    
             \Xhline{1\arrayrulewidth}
             FSB&   1,299,610&	2,574,093&	5,118,365&	10,203,006&	19,085,968&	25,428,308&	50,858,027&	76,281,332\\
             \Xhline{1\arrayrulewidth}
             PSE&   1,270,241&	2,540,883&	5,083,663&	10,174,162&	19,087,813&	25,459,164&	50,966,154&	76,475,320\\
             RND&   1,270,597&	2,541,622&	5,085,413&	10,174,783&	19,091,664&	25,463,114&	50,974,872& 76,482,020\\
             GCNN&  1,270,714&	2,541,293&	5,083,012&	10,169,973&	19,079,542&	25,449,533&	50,947,389&	76,457,625\\
             \Xhline{2\arrayrulewidth}
             GAT&1,271,428&	2,543,471&	5,088,825&	10,181,487&	19,097,850&	25,469,554	&50,968,796&	76,478,412\\

             TGAT&  1,271,488&	2,543,805&	5,089,730&	10,183,617&	19,103,078&	25,476,085&	50,982,813&	76,498,953
        \end{tabular}
    \end{tabular}
    \caption{Dual Integral Reward for Capacitated Facility Location Dataset}
    \label{tab:reward_facilities}
}
\end{table}
\endgroup
